Node Sampling using Random Centrifugal Walks

Sampling a network with a given probability distribution has been identified as a useful operation. In this paper we propose distributed algorithms for sampling networks, so that nodes are selected by a special node, called the \emph{source}, with a given probability distribution. All these algorithms are based on a new class of random walks, that we call Random Centrifugal Walks (RCW). A RCW is a random walk that starts at the source and always moves away from it. Firstly, an algorithm to sample any connected network using RCW is proposed. The algorithm assumes that each node has a weight, so that the sampling process must select a node with a probability proportional to its weight. This algorithm requires a preprocessing phase before the sampling of nodes. In particular, a minimum diameter spanning tree (MDST) is created in the network, and then nodes' weights are efficiently aggregated using the tree. The good news are that the preprocessing is done only once, regardless of the number of sources and the number of samples taken from the network. After that, every sample is done with a RCW whose length is bounded by the network diameter. Secondly, RCW algorithms that do not require preprocessing are proposed for grids and networks with regular concentric connectivity, for the case when the probability of selecting a node is a function of its distance to the source. The key features of the RCW algorithms (unlike previous Markovian approaches) are that (1) they do not need to warm-up (stabilize), (2) the sampling always finishes in a number of hops bounded by the network diameter, and (3) it selects a node with the exact probability distribution.

==> larger-distances.tex <==
\section{Sampling in a Concentric Rings Network with Uniform 
Connectivity at Distance 2}
\label{s:largerdistances}
%\subsection{Uniform connectivity}
In this section we generalize RCW to allow that each node could have neighbors at different distances from it, instead of having neighbors only at distance $1$. Intuitively, this enhancement  will reduce on average the number of steps taken in each random walk.
%RCW algorithm also works on networks, based on {\em Concentric Topologies} , but instead of nodes have neighbors at distance $1$, they can have neighbors at other distances ($1.. R$).
We study in this section networks where each node has neighbors at distances $1$ and $2$. As in the previously, we assume that two nodes in ring $k$ have the same number of neighbors in rings $k-2$, $k-1$, $k+1$, and $k+2$. Also, as before they have at least one neighbor in the rings at distance 1.

%Generalization for larger distances can be done using the same recurrent formula that we propose in the following paragraphs.

%We define in a node $x$ at a ring $i$, $k_{i,1}$ and $k_{i,2}$ as the number of neighbors that the node $x$ has at distances $1$ and $2$ respectively.
%\begin{itemize}
%\item from a node at ring $i$ we can link $k_{i,1}$ and $k_{i,2}$ neighbors at rings $i+1$ and $i+2$ respectively
%\item RCW algorithm can visit a node at ring $i$ from $l_{i,1}$ and $l_{i,2}$ nodes at rings $i-1$ and $i-2$ respectively.
%\end{itemize}

In this case a node in ring $k$ that receives the RCW and is not selected has to decide whether to send the walk to a neighbor at distance 1 or at distance 2 (among the neighbors at each distance it uses uniform probability). To decide on this, we use a parameter $s_k \in (0,1]$ that is the probability of choosing a neighbor at distance 1. The set of values $s_k$ has to be
large enough so that the desired probability distribution can be achieved (in particular, it must guarantee that the visit probability $v_k$ is no smaller than the selection probability $p_k$).

As in Section \ref{s:uniform}, the stay probability is set to $q_k=p_k/v_k$. The expression to compute $v_k$ now depends on parameters that can come from two rings away, as
\begin{multline}
v_k n_k = v_{k-1} n_{k-1} (1 - q_{k-1}) s_{k-1} + 
\\
v_{k-2} n_{k-2}(1-q_{k-2}) (1-s_{k-2}).
\end{multline}

Replacing the value of $q_{k-1}$ and $q_{k-2}$, we get
\begin{multline}
$$
v_k  = \frac{n_{k-1} (v_{k-1} - p_{k-1}) s_{k-1} + n_{k-2} (v_{k-2}-p_{k-2}) (1-s_{k-2})}{n_k}.
$$
\end{multline}
This is the expression that is used in Line 3 of the algorithm of Figure \ref{f-drw}. In addition to this change, the RCW, when sent to a node at ring $k$, must contain the values this node needs to compute $v_k$, namely $n_{k-1}$,  $v_{k-1}$, $p_{k-1}$, $s_{k-1}$,  $n_{k-2}$,  $v_{k-2}$, $p_{k-2}$,  and $s_{k-2}$. If the message is sent to a distance of 2, the sender (at ring $k-2$) must compute those values that it may not know (like $v_{k-1}$) before sending it. 

The initial values sent by the source are $v_0 = 1$, $p_0=0$, $n_0=1$, $v_{-1} = 0$, $p_{-1} =0$, $n_{-1} =0$, and fix $s_0=1$ (so the initial hop is always of length 1).
The proof that the algorithm obtained correctly computes the visit probabilities and hence
samples with the right probability distribution is similar to the one done in Section \ref{s:uniform} (provided the values $s_k$ are appropriately chosen).


%

%We use the same definition of the probability of select one node $p_i$:
%$$
%\mathrm{Pr} [select \ x] = p_i = Pr [visit \ ring \ i] \times \frac{1}{n_i} \times q_i
%$$
%As we do in section~\ref{s:uniform}, we use a recurrent expression, in this case based on the $v_{i-1}$ and $v_{i-2}$ probabilities, to calculate the $v_i$ probability:
%%$$
%%\mathrm{Pr} [visit \ ring \ i] = v_i = Pr[visit \ ring \ i-1] \times \frac{k_{i-1,1}}{k_{i-1,1}+k_{i-1,2}} \times (1-q_{i-1}) 
%%$$
%%$$
%%+ \ Pr[visit \ ring \ i-2] \times \frac{k_{i-2,2}}{k_{i-2,1}+k_{i-2,2}} \times (1-q_{i-2})
%%$$

%%v_i = \mathrm{Pr} [visit \ ring \ i]

%\begin{equation}
%\label{k2}
%v_i =  v_{i-1} \times \frac{k_{i-1,1}}{k_{i-1}} \times B_{i-1} + v_{i-2} \times \frac {k_{i-2,2}}{k_{i-2}} \times B_{i-2}
%\end{equation}
%Let define $v_0 = 1$ and $v_{-1} = 0$.
%To clarify the formula, we define $k_i =  k_{i,1} + k_{i,2}$,   $B_i = \frac {v_i-n_i \times p_i}{v_i}$ and $S_i = \frac{k_{i,1}}{k_i}$.
%Therefore, the new expression of the probability of visit ring $i$ is:
%$$
%v_i=(v_{i-1}-n_{i-1} \times p_{i-1}) S_{i-1} + (v_{i-2}-n_{i-2} \times p_{i-2})  (1-S_{i-2})
%$$
%where $S_{i-1}$ and $S_{i-2}$ are the probabilities to decide which neighbor type should be used for the next step in the random walk. These probabilities may have a fixed value or be a function of the number of neighbors of each type.

%%This is the probability to use in the RCW algorithm.

%\subsection {Distributed algorithm}
%As shown in Eq. \ref{k2},  we need $v_{i-1}$ and $v_{i-2}$ to calculate $v_i$ probability value, so the distributed algorithm RCW (Fig. \ref{f-drw}, line 5) must be modified to accomplish this new situation. Two different cases can appear in a node $x$ at ring $i$: a) the next RCW step is done to a node $y$ at distance $1$. In this case, the node $x$ sends its $v_i$, and the previous $v_{i-1}$, which are processed respectively as $v_{i-1}$ and $v_{i-2}$, to node $y$ . b) the next RCW step is done to a node $y$ at distance $2$. In this case, node $x$ computes $v_{i+1}$ (using $v_i$ and $v_{i-1}$), and sends $v_{i+1}$  and $v_i$,  which are processed respectively as $v_{i-1}$ and $v_{i-2}$, to the node $y$.

%

%

%

%






==> non-uniform.tex <==
\section{Sampling in a Concentric Rings Network without  Uniform Connectivity}
\label{s:nonuniform}

In this section we assume again that the RCW is only sent to neighbors at distance 1, and we consider a realistic scenario in which the network does not satisfy uniform connectivity (i.e., Eq. \ref{satisfy_cond}). This fact makes harder to enforce the property that all nodes in a ring $k$ are visited with the same probability, since some have a large number of neighbors and others may have a smaller number. If nodes in ring $k-1$ choose the target of a RCW in ring $k$ uniformly, most possibly the visit distribution will be biased.
However, we will impose the following restriction, which is much simpler to satisfy. For each $k \in [1,R)$, it must hold that
\begin{equation}
\label{halls}
\frac{n_{k+1}}{n_k} \leq \frac{\min_{x \in \mathbb{R}_k} \delta_k(x)}{\max_{y \in \mathbb{R}_{k+1}} \gamma_{k+1}(y)}
\end{equation}

To preserve the property that visit probabilities are the same in each ring, nodes will use different probabilities for different neighbors. Instead of explicitly computing the probability for each neighbor, we will use the following process. Consider rings $k$ and $k+1$. Let $r=\mathit{LCM}(n_k,n_{k+1})$, where $\mathit{LCM}$ is the {\em least common multiple} function. 
We assign $\frac{r}{n_k}$ \emph{attachment points} to each node in ring $k$, and $\frac{r}{n_{k+1}}$ attachment points to each node in ring $k+1$. Now, the problem is to connect each
attachment point in ring $k$ to a different attachment point in ring $k+1$ (not necessarily in different nodes). If this can be done, we can use the algorithm of Figure \ref{f-drw} but when
a walk is sent to the next ring, an attachment point is chosen uniformly (instead of a neighbor). Since the number of attachments points is the same in all nodes of ring $k$ and in all nodes of ring $k+1$, the impact in the visit probability is that it is again the same for all nodes of a ring.

\begin{figure}[t]
%\begin{minipage}[t]{1\columnwidth}
%
\lstset{xleftmargin=15mm}
\begin{lstlisting}
function $\mathit{AssignAttachmentPoints} (x,k)$
$ap$:= $\frac{\mathit{LCM}(n_k,n_{k+1})}{n_k}$
$C$:=$\mathbb{N}_{k+1}(x)$    /* neighbors of $x$ in ring $k+1$ */
$A_x$:= empty list
loop
	choose $c$ from $C$
	$\mathit{send}$ $attach\_msg$ to $c$
	$\mathit{receive}$ $response\_msg$ from $c$ 
	if $response\_msg = ok$ then
		$ap$ := $ap - 1$
		append $c$ to $A_x$       /* $c$ can be in $A_x$ several times */
	else
		$C$ := $C \setminus \{c\}$
	end if
until $ap = 0$
return $A_x$
\end{lstlisting}
%
%\end{minipage}
\vspace{0,0em}
\caption{Assignment Attachment Points (AAP) Function.}
\label{AAP}
\end{figure}

The connection between attachment points can be done with a function like the one presented in Figure \ref{AAP}, in which a node $x$ in ring $k$ contacts its neighbors to request available  attachment points. If a neighbor that is contacted has some free attachment point, it replies with a response message accepting the connection. Otherwise it replies to $x$ notifying that all its attachment points have been connected. The node $x$ continues trying until its $\frac{r}{n_k}$ attachment points have been connected.
%
The property that is left to prove is that that function of Figure \ref{AAP} always finishes. To do so, we apply Hall's Theorem \cite{Hall:1935}. In our context, it says that, if for each subset $X$ of  $\mathbb{R}_k$ the number of attachment points of the neighbors in ring $k+1$ is at least as large as the number of attachment points in $X$, then a greedy connection process like the one done by function $\mathit{AssignAttachmentPoints}$ will always complete. 

Consider any set $X \subseteq \mathbb{R}_k$. The total number of attachment points of the nodes in $X$ is
$\frac{r|X|}{n_k}$. Let $Y$ be the set of neighbors of $X$ in ring $k+1$. The size of $Y$ is at least $|X| \frac{\min_{x \in \mathbb{R}_k} \delta_k(x)}{\max_{y \in \mathbb{R}_{k+1}} \gamma_{k+1}(y)}$. Each of the nodes in $Y$ has $\frac{r}{n_{k+1}}$ attachment points. Hence, from the property of Eq.~\ref{halls}, the number of attachment points in $Y$ is at least as large as the number of attachment points in $X$. Since this holds for all $X \subseteq \mathbb{R}_k$, Hall's Theorem can be applied to show the following lemma.

\begin{lemma}
Under the assumption of Eq.~\ref{halls}, if the nodes of ring $k$ execute the algorithm of Figure \ref{AAP} they will always complete it and be able to connect all their attachment points.
\end{lemma}

Combining these results with the analysis of Section~\ref{s:uniform}, we can conclude with the following theorem

\begin{theorem}
Using attachment points instead of links and the distributed RCW-based algorithm of Figure \ref{f-drw}, it is possible to sample a concentric rings network without  uniform connectivity with any desired distance-based probability distribution $p_k$, provided Eq.~\ref{halls} holds.
\end{theorem}

%
%So, the condition about adjacent rings connectivity (eq. \ref{satisfy_cond}) could not be fulfilled.
%%
%In this scenario, a node at ring $i$ could not be visited because it might not have any neighbor at ring $i-1$ connected with it, and also, a node at ring $i$ with no neighbors at ring $i+1$ could stop the RCW if it was visited. Therefore, it is necessary to design a correction mechanism to overcome this problem. 
%%
%To guarantee that the former scenarios do not happen, we define $r=LCM(n_i,n_{i+1})$ (LCM is the {\em least common multiple}), and we assign $\frac{r}{n_i}$ attachment points to neighbors at ring $i+1$, to each node at ring $i$, and $\frac{r}{n_{i+1}}$ attachment points to neighbors at ring $i+1$,  to each node at ring $i$. With this assignment the following condition is fulfilled, 
%$$
%\forall \ x \subseteq \mathbb{R}_i \, \, , \, \, \, \delta_{i} \cdot n_i \ge n_{i+1}
%$$
%and hence the {\em marriage condition} of  Hall's Theorem \cite{Hall:1935} is satisfied. 
%This condition allows the existence of at least one possible match between the nodes of ring $i$ with the nodes of ring $i+1$, where no node is unattached. Therefore, the former adjacent rings connectivity condition (eq. \ref{satisfy_cond}) is now fulfilled and the later problematic scenarios are not possible.

%Finally, we propose in Fig. \ref{AAP} a distributed algorithm to make the assignment of the attachment points to each network node $x$ at ring $i$, knowing $n_i$, $n_{i+1}$ and $\mathbb{R}_i$.



==> nuevademo.tex <==
\section{RCW sampling demo}

Let us denote $\eta_s = \sum_{\substack{j \in N\\j \ne s}} w(j)$.  Then, the probability of selecting $x \in N$ from a source $s$ is $p_s(x)=w(x)/\eta_s$. 


\begin{theorem}
\label{d-drw-spt}
Each node $x \in N$ is visited by the RCW, from a source $s$,  with probability $v_s(x)=\frac{T_s(x)}{\eta_s}$ and selected by the RCW algorithm with probability $p_s(x)=\frac{w(x)}{\eta_s}$.
\end{theorem}

\begin{proof}
We prove the claim by induction on the number of hops from the source $s$ to node $x$ in the spanning tree.
The base case is when the node $x$ is at $1$ hop of $s$ (i.e., it is a child of $s$). Then, $x$ is visited with probability $\frac{T_s(x)}{\eta_s}$,
since $x$ is chosen by $s$ with this probability in the first hop of the RCW (Observe that $q_s(x) = 0$, when $x = s$).
If $x$ is visited, then it is selected (i.e., RCW stops) with probability $q_s(x) = \frac{w(x)}{w(x)+\sum_{j \in candidates(x)} T_s(j)} = \frac{w(x)}{T_s(x)}$. Then, the probability of being selected is

$$
\mathrm{Pr} [\mathrm{select}\ x \ \mathrm{from\ source}\ s] = \frac{T_s(x)}{\eta_s}\frac{w(x)}{T_s(x)}=\frac{w(x)}{\eta_s}.
$$
where
$$
T_s(x) = w(x)+\sum_{i \in candidates(x)} T_s (i)
$$
$$
\eta_s = \sum_{i \in neighbors (s)} T_s (i)
$$



The induction hypothesis assumes the claim true for a node $x$ at distance $i$ from $s$. We consider a child $y$ of $x$,
which is at distance $i+1$ from $s$.
$$
\mathrm{Pr} [\mathrm{visit}\ y \  \mathrm{from}\ s] = v_s(x) \left(1-q_s(x)\right)\frac{T_s(y)}{\sum_{j \in candidates (x)}T_s(j)}
$$
$$
\mathrm{Pr} [\mathrm{visit}\ y \  \mathrm{from}\ s] = v_s(x) \left(1-q_s(x)\right)\frac{T_s(y)}{T_s(x)-w(x)},
$$
where $1-q_s(x)$ is the probability of not staying at node $x$ from source $s$, and $\frac{T_s(y)}{T_s(x)-w(x)}$ 
is the probability to choose the child node $y$ from source $s$ in the next hop of the RCW. Then,
$$
v_s(y)  =  \frac{T_s(x)}{\eta_s}\left(1-\frac{w(x)}{T_s(x)}\right)\frac{T_s(y)}{T_s(x)-w(x)} 
$$
$$
v_s(y)  = \frac{T_s(x)}{\eta_s} \left(\frac {T_s(x) - w(x)}{T_s(x)}\right) \frac{T_s(y)}{T_s(x)-w(x)} 
= \frac{T_s(y)}{\eta_s}.
%\begin{eqnarray*}
%v(y) & = & \frac{T(x)}{\eta}\left(1-\frac{w(x)}{T(x)}\right)\frac{T(y)}{T(x)-w(x)} 
%&=& \frac{T(x)}{\eta} \left(\frac {T(x) - w(x)}{T(x)}\right) \frac{T(y)}{T(x)-w(x)} 
%&=& \frac{T(y)}{\eta}.
%\end{eqnarray*}
$$
and
$$
\mathrm{Pr} [\mathrm{select}\ y \ \mathrm{from\ source}\ s] = v_s(y) q_s(y) = \frac{T_s(y)}{\eta_s}\frac{w(y)}{T_s(y)}=\frac{w(y)}{\eta_s}.
$$
\end{proof}


==> su-simulations.tex <==
\section{Concentric Rings Networks without Uniform Connectivity}
\label{s:sum-simulations}

%We have previously presented a RCW algorithm on concentric rings networks with uniform connectivity. 
%This algorithm has no need of preprocessing or storing information in the network nodes as it happens in the connected networks.
Finally, we are interested in evaluating by means of simulations the performance of RCW algorithm when it is used on a more realistic topology: a concentric rings network without uniform connectivity. The experiment has been done in a concentric rings topology of $100$ rings with $100$ nodes per ring, and it places the nodes of each ring uniformly {\em at random} on each ring and  all the nodes use the same predefined connectivity angle to find neighbors. Remember that every node must have neighbors in the next ring to avoid stopping a RCW for absence of neighbors to jump to. We compare the relative error of the RCW algorithm when sampling with two distributions: the uniform distribution (UNI) and a distribution proportional to the inverse of the distance (PID). 

The simulation results show a biased behavior of RCW algorithm because the condition of Eq.~\ref{satisfy_cond} is not fulfilled in this experiment (i.e. a node has no neighbors, or there are two nodes in a ring $k$ that have different number of neighbors in rings $k-1$ or $k+1$). 
To eliminate these errors observed when there is no uniform connectivity, we propose a simple algorithm to transform the concentric rings network without uniform connectivity into an overlay network with uniform connectivity. 
To preserve the property that the visit probability is the same for all the nodes in a ring, nodes will use different probabilities for different neighbors. Instead of explicitly computing the probability for each neighbor, we will use the following process. Consider rings $k$ and $k+1$. Let $r=\mathit{LCM}(n_k,n_{k+1})$, where $\mathit{LCM}$ is the {\em least common multiple} function. 
We assign $\frac{r}{n_k}$ \emph{attachment points} to each node in ring $k$, and $\frac{r}{n_{k+1}}$ attachment points to each node in ring $k+1$. Now, the problem is to connect each
attachment point in ring $k$ to a different attachment point in ring $k+1$ (not necessarily in different nodes). If this can be done, we can use RCW algorithm of Figure \ref{f-drw}, but when a RCW is sent to the next ring, an attachment point is chosen uniformly (instead of a neighbor). Since the number of attachments points is the same in all nodes of ring $k$ and in all nodes of ring $k+1$, the impact in the visit probability is that it is again the same for all nodes of a ring.
The connection between attachment points can be done with the simple distributed algorithm \emph{Assignment Attachment Points} (AAP) presented in \cite{RCWarxiv}.
Therefore, when nodes are placed uniformly at random and AAP is used to attach neighbors to each node, the average relative error of RCW is nearly equal to the obtained with the UNI or PID simulators.
All the details and results of this experiment and the description of the AAP algorithm can be found in \cite{RCWarxiv}.

%In this section we explore this line by means of simulations.

%\subsection{Evaluation Environment}
%\paragraph{Evaluation Environment}

%We compare the relative error of the RCW algorithm when sampling with two distributions: the uniform distribution and a distribution proportional to the inverse of the distance (PID).  We define the relative error $e_i$ for a node $x$ in a collection $C$ of $s$ samples as $e_i=\frac{|fsim_x - f_x|}{f_x}$, where $fsim_x$ is the number of instances of $x$ in collection $C$ obtained by the simulator, and $f_x= p_x \cdot s$ is the expected number of instances of $x$ with the ideal probability distribution (uniform or PID). We compare the error of the RCW algorithm with the error of a generator of pseudorandom numbers.

%The experiment has been done in a concentric rings topology of $100$ rings with $100$ nodes per ring. For the experiment, a collection of $10^7$ samples has been obtained, in order to guarantee that every node appears on average $1000$ times (with the uniform distribution). 

%We have used two different node configurations in our experiments. Firstly, we only assign neighbors at distance $1$ to each node, and secondly we assign neighbors at different distances ($1$ and $2$) to each node. Intuitively, we obtain on average, shorter random walk lengths when there are neighbors at larger distances.

%In order to establish the connectivity of nodes, we do a geometric deployment. A node $x$ in ring $k$ is assigned a position in the ring.
%This position can be given by an angle $\alpha$. Then, each network studied will have associated a connectivity angle $\beta$.
%This means that $x$ will be connected to all the nodes in rings $k-1$ and $k+1$ 
%(and maybe at those at distance 2 as well) whose position (angle) is in the interval $[\alpha-\beta/2, \alpha+\beta/2]$.

%We have define two experiments, placing the nodes of each ring in two different ways: (experiment 1) uniformly on each ring (fixed angle between nodes), 
%The first experiment results in a concentric rings network with uniform connectivity. 
%The second does not guarantee uniform connectivity, but should be close to it. If the performance of both experiments is very different,that will imply that the RCW algorithm for uniform connectivity cannot be used if that property is not satisfied.
%In this experiment we have run scenarios with a uniform distribution, and with a PID distribution. 

%The experiment places the nodes of each ring uniformly {\em at random} on each ring and  all the nodes use the same predefined connectivity angle to find neighbors. Remember that every node must have neighbors in the next ring to avoid stopping a RCW for absence of neighbors to jump to. 
%When placing nodes uniformly on each ring, it is enough to have a fairly small angle (inversely proportional to the nodes' density in the rings) to satisfy this.
%Note that the connectivity angle can be as large as $360^{\circ}$ to satisfy the property (\ref{satisfy_cond}).

%\subsection{Results of the Experiments}
%\paragraph{Results of the Experiment}

%We describe now the observed behavior of the algorithms and simulators in the different scenarios.

%\paragraph{Experiment 1} In this experiment the nodes are uniformly placed in each ring. The left side of Figure \ref{fig:E1-1} presents the uniform sampling scenario, where we show the average values of the relative error for the RCW simulator, when configured with neighbors only at distance $1$ (RCW-K1), with neighbors at distances $1$ and $2$ (RCW-K2), and when a uniform distribution simulator (UNI) based on a pseudorandom generator is used, to compare the results. As expected, it can be observed that the average relative errors obtained with RCW-K1 and RCW-K2 (independently of the connectivity angle used) are the same as the average relative error of the UNI simulator.
%The right side of Figure \ref{fig:E1-1} shows the PID sampling scenario. We can see again a similar behavior of RCW-K1 and RCW-K2 when compared with the PID simulator.

%In this experiment the nodes are placed uniformly at random in each ring. The left side of Figure \ref{fig:E1-2} presents the uniform sampling scenario and the right side presents the PID scenario. In both cases, when using RCW-K1 and RCW-K2,  we can see worse results than with the UNI and PID simulators. This is mainly due to the fact that there are nodes without neighbors in the next ring except when large angles ($\ge180^{\circ}$) are used.


